A Survey for Federated Learning Evaluations: Goals and Measures

Evaluation is a systematic approach to assessing how well a system achieves its intended purpose. Federated learning (FL) is a novel paradigm for privacy-preserving machine learning that allows multiple parties to collaboratively train models without sharing sensitive data. However, evaluating FL is challenging due to its interdisciplinary nature and diverse goals, such as utility, efficiency, and security. In this survey, we first review the major evaluation goals adopted in the existing studies and then explore the evaluation metrics used for each goal. We also introduce FedEval, an open-source platform that provides a standardized and comprehensive evaluation framework for FL algorithms in terms of their utility, efficiency, and security. Finally, we discuss several challenges and future research directions for FL evaluation.

==> sections/response.tex <==
\noindent
\textbf{Paper}: TKDE-2023-08-1161

\noindent
\textbf{Title}: A Survey for Federated Learning Evaluations: Goals and Measures

\noindent
\textbf{Authors}: Di Chai, Leye Wang, Liu Yang, Junxue Zhang, Kai Chen, and Qiang Yang

\vspace{0.5cm}

\noindent
Dear Editor and Reviewers,

\vspace{0.25cm}
\noindent
Thanks for your insightful and constructive comments and advice. We have carefully addressed these concerns and appropriately revised the manuscript. These comments and suggestions have enabled us to provide a highly improved manuscript. We really appreciate your help in processing this paper, and we are looking forward to hearing from you soon.

\vspace{0.25cm}
\noindent
Yours sincerely,

%\vspace{0.2cm}
\noindent
Di Chai and Leye Wang

\vspace{0.2cm}
\noindent \rule[1px]{6cm}{0.05em}
\vspace{0.2cm}

\noindent
Below, we first summarize all changes made to the manuscript in the revision. Then, we list all the responses to the comments made by each reviewer.

\section*{Summary of Changes} 
% \begin{cmt*}{}{}
% Editor Comments.
% \end{cmt*}

% \vspace{0.1cm}
% \noindent
% \underline{\textbf{Response:}}
% \vspace{0.2cm}

% Your response. 

\vspace{0.1cm}
\noindent \Cref*{sec:introduction} - Introduction
\vspace{0.1cm}
\begin{enumerate}
    \item \highlight{Enrich necessary backgrounds including workflow of FL and its multiple objectives.}
    \item \highlight{Explain the challenge of appropriate evaluation in FL.}
    \item \highlight{Demonstrate the issues of inappropriate evaluation in FL using examples.}
\end{enumerate}

\vspace{0.3cm}
\noindent \Cref*{sec:goals} - Federated Learning Evaluation Goals
\vspace{0.1cm}
\begin{enumerate}
    \item \highlight{Add the necessity and challenge of doing a comprehensive evaluation.}
    \item \highlight{Discuss solutions to reduce the workload of comprehensive evaluation.}
\end{enumerate}

\vspace{0.3cm}
\noindent \Cref*{sec:measure} - Federated Learning Evaluation Measures
\vspace{0.1cm}
\begin{enumerate}
    \item \highlight{Explain the rationale of utility definition.}
    \item \highlight{Reorganize the structure of this section.}
    \item \highlight{Reformat \Cref*{tab:utility,tab:efficiency metrics,tab:privacy} and enrich information to illustrate the characteristics of each paper.}
\end{enumerate}

\vspace{0.3cm}
\noindent \Cref*{sec:fedeval} - FedEval: A platform for FL System Evaluation
\vspace{0.1cm}
\begin{enumerate}
    \item \highlight{Enrich the details of the FedEval platform (\eg, the methods to produce standardized evaluations that are close to real-world conditions).}
    \item \highlight{Add utility evaluation results (\ie, \Cref*{tab:utility evaluation}).}
    \item \highlight{Enrich analysis showing the evaluation produced by FedEval matches the original paper.}
    \item \highlight{Analyze the limitations of FedEval and the corresponding solutions.}
\end{enumerate}

\vspace{0.3cm}
\noindent \Cref*{sec:conclusion} - Conclusion
\vspace{0.1cm}
\begin{enumerate}
    \item \highlight{Enrich the conclusion to better summarize the work done in this paper.}
\end{enumerate}

% \fbox{\begin{minipage}{0.9\textwidth}\revision{Evaluation plays a critical role in designing various FL algorithms and systems, owing to the need for rigorous performance assessment, providing comparative analysis between different algorithms, ensuring robustness across diverse environments, and identifying limitations for further improvement.}\end{minipage}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Rewiewer 1
\newpage
\section{Response to Reviewer 1} 

%%%%%%%%%%%%%
\noindent
\underline{\textbf{Comment 1:}} \textbf{In the introduction, there is less background related to the content of this article. Please enrich the relevant research background in the introduction.}

\vspace{0.3cm}
\noindent
\underline{\textbf{Response:}} Thanks for your valuable suggestion. We have updated the introduction (\Cref*{sec:introduction}) to enrich the relevant research backgrounds, including 1) adding the workflow of FL; 2) emphasizing the importance of evaluation in FL and its challenges; and 3) demonstrating the issue of inappropriate evaluation in FL. Specifically, the revision includes:

\begin{enumerate}
    \item \textbf{Paragraph 2.} We highlight the necessity of appropriate evaluation in FL. Specifically, evaluation plays a critical role in designing various FL algorithms and systems, owing to the need for rigorous performance assessment, providing comparative analysis between different algorithms, ensuring robustness across diverse environments, and identifying limitations for further improvement.
    \item \textbf{Paragraph 3.} We introduce the workflow of FL and explain why evaluation of FL is challenging. Specifically, 1) we introduce a typical FL workflow consisting of three steps, including uploading updates, server aggregation, and retrieving the latest model; b) we emphasize the evaluation of FL is challenging since FL is a cross-domain topic that has multiple objectives; c) we analyze the tradeoff between the multiple objectives, and it is hard to design one solution with optimized performance on all objectives.
    \item \textbf{Paragraph 5.} We demonstrate the issues of inappropriate evaluation in FL. Specifically, 1) inappropriate privacy evaluation may cause leakage of privacy data in the application and decrease people's trust and willingness to further contribute data to the federation; 2) inappropriate utility evaluation may cause poor model performance since the data distribution is highly heterogeneous in the real-world application; 3) inappropriate efficiency evaluation, \eg, not evaluated on real-world networking conditions, cause low-efficiency issues in the real-world application.
\end{enumerate}

%%%%%%%%%%%%%
\vspace{0.3cm}
\noindent
\underline{\textbf{Comment 2:}} \textbf{This paper has some grammar errors and some sentences do not read smoothly which should be checked by authors to make it more understandable to the readers. Please correct these.}

\vspace{0.3cm}
\noindent
\underline{\textbf{Response:}} Thanks for your valuable suggestion. We have carefully checked the writing of the paper and corrected the grammar issues as well as the unclear sentences.

\vspace{0.3cm}
\noindent Examples of fixing the grammar issues and rewriting sentences to improve clarity.
\begin{mdframed}[style=2]
\textbf{Before revision}: FL models that demonstrate excellent performance are preferable for real-world deployments, while those with significant issues such as private data leakage are not suitable for practical applications.

\noindent
\textbf{Rewrite for clarity}: \highlight{Real-world applications prefer FL models with excellent performance. FL models with significant issues, such as private data leakage, are unsuitable for practical applications.}

\vspace{0.3cm}
\noindent \textbf{Before revision}: In this survey, we will begin by summarizing the evaluation
goals of FL.

\noindent
\textbf{Rewrite for clarity}: \highlight{In this survey, we first summarize the evaluation goals for FL.}

\vspace{0.3cm}
\noindent \textbf{Before revision}: The evaluation goals and measures presented in this survey does not restrict the type of FL and work with both HFL and VFL.

\noindent \textbf{Grammar issue:}: The evaluation goals and measures presented in this survey \highlight{do} not restrict the type of FL and work with both HFL and VFL.

\noindent ...

\end{mdframed}

%%%%%%%%%%%%%
\vspace{0.5cm}
\noindent
\underline{\textbf{Comment 3:}} \textbf{As an open-source platform, FedEval can provide a comprehensive evaluation framework for the practicability, efficiency and security of FL algorithm, but does it have limitations? How to solve it?}

\vspace{0.3cm}
\noindent
\underline{\textbf{Response:}} Thanks for your valuable suggestion. In \Cref*{sec:fedeval}, we analyze the limitations of FedEval and the corresponding further work to solve these limitations. Specifically, FedEval has two limitations. First, while the platform provides good support for utility and efficiency evaluations, the privacy and security evaluation attacks still need to be enriched. Second, the evaluation of vertical FL algorithms is currently not supported by FedEval. We will keep updating the platform to solve these two limitations by adding more attacks regarding privacy and security evaluation and adding support for the evaluation of vertical FL. Specifically, the following revision is added to \Cref*{sec:fedeval}:

\begin{mdframed}[style=2]
In summary, FedEval provides a flexible framework for researchers to produce standardized evaluation results that closely mimic real-world settings using the measurements summarized in this survey. FedEval also reduces the workload required for comprehensive analysis since researchers only need to define the FL workflow (\ie, through scripts), and evaluations can be automatically completed using the built-in metrics on the platform. 
\highlight{While being a platform that makes a significant contribution to the evaluation of FL, FedEval also has two limitations. Firstly, while the platform provides good support for utility and efficiency evaluations, the attacks for privacy and security evaluation still need to be enriched. Secondly, the automated evaluation of vertical FL algorithms is currently not supported by FedEval. We will keep updating the platform in the future to solve these two limitations, \ie, adding more attacks regarding the privacy and security evaluation and adding support for the evaluation of vertical FL.}
\end{mdframed}

%%%%%%%%%%%%%
\vspace{0.5cm}
\noindent
\underline{\textbf{Comment 4:}} \textbf{In the conclusion part, the work done in this paper should be described in more detail.}

\vspace{0.3cm}
\noindent
\underline{\textbf{Response:}} Thanks for your valuable suggestion. We enrich the conclusion section (i.e., Section VI) to describe the work done in this paper in detail. Specifically, the following is the enriched conclusion part.

\begin{mdframed}[style=2]\highlight{In this survey, we provide a comprehensive overview of the evaluation goals and measures for FL studies. We categorized the key evaluation goals into utility, efficiency, and security \& privacy. For each goal, we reviewed commonly used metrics and evaluation methods from existing literature. We also discussed the necessity of conducting comprehensive evaluations across all goals due to the trade-offs between them. To facilitate such comprehensive analysis, we introduced FedEval, an open-source platform that simplifies implementing standardized FL evaluations.}\end{mdframed}

%%%%%%%%%%%%%
\vspace{0.5cm}
\noindent
\underline{\textbf{Comment 5:}} \textbf{The format of the references is problematic and should be revised.}

\vspace{0.3cm}
\noindent
\underline{\textbf{Response:}} Thanks for your valuable suggestion. We have carefully checked and updated all the references, including unifying the formats and updating the out-of-date references. Specifically, we update all the references following the condensed format from dblp.org.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Rewiewer 2
\section{Response to reviewer 2}

%%%%%%%%%%%%%
\noindent
\underline{\textbf{Comment 1:}} \textbf{The authors over-emphasize the "comprehensive" goals or evaluation of FL systems, as the comprehensive evaluation of FL systems (FedEval) is not well motivated. Most of the works commonly deal with just one or two goals, i.e., utility, efficiency, or security \& privacy. The aims of these works are different. Scant research works are devoted to improving all three goals. Accordingly, there is no need to evaluate or compare the FL systems in multiple dimensions (as in Fig. 4).}

\vspace{0.3cm}
\noindent
\underline{\textbf{Response:}} Thanks for your valuable suggestion. We agree with the reviewer that most works have just one or two goals. Thus, they have limited motivation to evaluate all the goals. However, even under such circumstances, a comprehensive evaluation can still be beneficial for researchers who want to conduct future research based on the proposed technique, as well as engineers who are trying to use the proposed technique in practice. For example, suppose one new FL algorithm significantly improves the efficiency. In that case, it is beneficial to check other targets (\ie, utility and, security \& privacy) to determine whether the new algorithm is a huge breakthrough (\ie, improving efficiency without affecting the other goals) or just another trade-off (\ie, improving efficiency while harming the utility or security \& privacy). To address this comment clearly, we add one subsection in \Cref*{sec:goals} to demonstrate the benefits and necessity of a comprehensive evaluation. Specifically, a comprehensive evaluation is a) the foundation of fair comparisons and b) the key to finding all the limitations before being applied in real-world applications.

In brief, we totally agree with the reviewer that one paper does not necessarily improve all the dimensions of FL systems. However, a comprehensive evaluation may still be useful as it can test whether other dimensions are degraded or not while improving a certain focused dimension of FL systems.

We understand the reviewer's concern about comprehensive evaluation might come from the workload, \ie, doing a comprehensive evaluation on all goals requires a significant workload. To solve this concern, we propose two solutions: 1) We develop a standardized evaluation platform, FedEval, to produce comparable and comprehensive results while reducing evaluation workload; 2) For incremental methods that only improve one or two goals based on an existing solution, another option is to analyze that the remaining goals have identical performance to prior studies that already reported comprehensive evaluation results. 

\vspace{0.3cm}
\noindent
The corresponding revision of this comment in \Cref*{sec:goals}:
\begin{mdframed}[style=2]
\highlight{
Based on our survey, we highly recommend new FL algorithm or systems to perform a comprehensive analysis on all the goals, including security and privacy, utility, and efficiency, for two reasons: 1) comprehensive analysis is the foundation of a fair comparison, and 2) comprehensive analysis is the key to find all the limitations before applied in real-world applications. Specifically, the comparison between different FL studies on partial goals is unfair because different goals form trade-offs and superiority in partial goals does not mean superiority in all goals. For instance, many works do not analyze privacy protection, which will bring unfair efficiency comparisons. Because FL algorithms' efficiency varies greatly under different privacy-protection methods. For example, differential privacy (DP) and homomorphic encryption (HE) employ different privacy mechanisms and have very different efficiencies. However, claiming the DP-based method is much more efficient than the HE-based method as a major innovation is problematic without understanding their relative privacy guarantees. The major disadvantage of DP is that it harms model utility while HE does not. Comprehensive analysis is also essential to thoroughly assess one algorithm or system and discover all the limitations, such that the issue (\eg, privacy or efficiency problems) could be fixed before being applied in real-world applications.

The major challenge of performing comprehensive analysis is the workload required for evaluations. To address this, we propose two solutions: 1) We develop a standardized evaluation platform, FedEval, to produce comparable and comprehensive results while reducing evaluation workload, and the detailed is introduced \Cref*{sec:fedeval}; 2) For incremental methods that only improve one or two goals based on an existing solution, another option is to analyze that the remaining goals have identical performance to prior studies that already reported comprehensive evaluation results. However, if the remaining goals were also not previously evaluated, assessments across all goals remain necessary.
}
\end{mdframed}

% \fbox{\begin{minipage}{0.9\textwidth}\highlight{#1}\end{minipage}}

%%%%%%%%%%%%%
\vspace{0.5cm}
\noindent
\underline{\textbf{Comment 2:}} \textbf{While the authors simplify the consequences of an unreasonable evaluation process by using only a medical accident as an example in the Introduction. As an evaluation survey, it still fails to emphasize the significance of the evaluation process in corresponding research and its importance in both theoretical and practical aspects.}

\vspace{0.3cm}
\noindent
\underline{\textbf{Response:}} Thanks for your valuable suggestion. We revise the \Cref*{sec:introduction} to emphasize the importance of FL evaluation in both theoretical and practical aspects: 1) theoretically, only appropriate and comprehensive evaluation can fully reveal the tradeoffs between different objectives, as well as the theoretical upper and lower bounds on the performance of different methods under varying conditions (\eg, different data distributions). A clear understanding of the tradeoffs provides us guidelines for finding future research directions in FL; 2) practically, appropriate and comprehensive evaluation is crucial to promote the healthy development of FL applications regarding identifying any critical issues before applying to real-world systems.

Specifically, we enrich the following paragraphs of \Cref*{sec:introduction} (introduction) to emphasize the importance of FL evaluation:
\begin{itemize}
	\item \textbf{Paragraph 2.} From the big picture, we emphasize that evaluation plays a crucial role in federated learning to fairly assess and compare algorithm performance, as well as validate the robustness and limitations in real-world scenarios.
	\item \textbf{Paragraph 3.} From the theoretical perspective, we show that the evaluation of FL is challenging since FL has multiple objectives that form tradeoffs \cite{NFL-1,NFL-2}. Appropriate and comprehensive evaluations can guide our future research directions by fully revealing the tradeoffs between different objectives, as well as the theoretical upper and lower bounds on the performance of different methods under varying conditions (\eg, different data distributions). 
	\item \textbf{Paragraph 4\&5.} From the practical perspective, we show that inappropriate evaluation will produce biased assessments, and the undiscovered limitations in FL algorithms or systems will damage real-world applications. And appropriate evaluation itself can have various applications, \eg, working as quality control for real-world applications.
\end{itemize}

% from the following aspects: 1) evaluation plays a critical role in designing FL algorithms and systems to provide rigorous and comparable performance assessment; 2) evaluation of FL is challenging due to tradeoff between FL's multiple objectives; 3) we demonstrate the benefit of appropriate evaluation and issues brought by inappropriate evaluations. Specifically, the changes to \Cref*{sec:introduction} include

% \begin{enumerate}
%     \item \textbf{Paragraph 2.} Evaluation plays a critical role in designing various FL algorithms and systems, owing to the need for rigorous performance assessment, providing comparative analysis between different algorithms, ensuring robustness across diverse environments, and identifying limitations for further improvement.
%     \item \textbf{Paragraph 3.} The evaluation of FL is challenging as it is a multi-objective and cross-domain research topic that leverages techniques from machine learning, distributed systems, cryptography, \etc. Enhancing one target usually has negative impacts on the other targets~\cite{NFL-1,NFL-2}. For example, increasing the number of local updates before global synchronization (\ie, reducing global synchronization frequency) can improve communication efficiency but harm model accuracy (\ie, caused by the non-IID issue). Thus, a well-designed evaluation is essential to produce rigorous and comparable evaluation results.
%     \item \textbf{Paragraph 4.} Appropriate evaluation is crucial to promote the healthy development of FL, and the evaluations themselves can enable further applications, e.g., working as quality control for real-world applications, working as a contribution evaluation method in incentive mechanism, and working as an online verification system during FL training.
%     \item \textbf{Paragraph 5.} Inappropriate evaluation will produce biased assessments, and the undiscovered limitations in FL algorithms or systems will damage real-world applications. For example, undiscovered privacy vulnerabilities will not only leak data providers' privacy but also decrease people's trust and willingness to further contribute data in the federated systems; FL algorithms untested under different data distributions may achieve poor model quality in applications as the data distribution in real-world applications can be highly heterogeneous; FL systems not evaluated on real-world network conditions may fail to achieve expected efficiency in applications due to the limited bandwidth and high latency in real-world applications.
% \end{enumerate}

The corresponding revision of this comment in \Cref*{sec:introduction}:

Paragraph 2.

\fbox{\begin{minipage}{0.9\textwidth}\highlight{Evaluation plays a critical role in designing various FL algorithms and systems, owing to the need for rigorous performance assessment, providing comparative analysis between different algorithms, ensuring robustness across diverse environments, and identifying limitations for further improvement.} Conceptually, evaluation is a systematic method to...\end{minipage}}

\vspace{0.1cm}
Paragraph 3.

\fbox{\begin{minipage}{0.9\textwidth}\highlight{The evaluation of FL is challenging as it is a multi-objective and cross-domain research topic that leverages techniques from machine learning, distributed systems, and cryptography, \etc.} ... \\\highlight{Generally, studies from the machine learning domain aim to improve the model utility, studies from distributed systems aim to improve efficiency, and privacy-preserving researchers mainly focus on privacy protections. Existing studies~\cite{NFL-1,NFL-2} have shown that these targets are not independent objectives and exhibit substantial interrelation. Enhancing one target usually has negative impacts on the other targets~\cite{NFL-1,NFL-2}. For example, increasing the number of local updates before global synchronization (\ie, reducing global synchronization frequency) can improve communication efficiency but harm model accuracy. With more local updates, a model trained on heterogeneous, non-identical-and-independent distributed (non-IID) data across clients will deviate further from the global optimum, which is known as the non-IID issue~\cite{zhao2018federated}. This illustrates the trade-off between communication efficiency and model utility, and we will discuss more trade-offs between different targets in \Cref*{sec:tradeoff}. Appropriate and comprehensive evaluations can guide our future research directions by fully revealing the tradeoffs between different objectives, as well as the theoretical upper and lower bounds on the performance of different methods under varying conditions (\eg, different data distributions).}\end{minipage}}

\vspace{0.1cm}
Paragraph 4.

\fbox{\begin{minipage}{0.9\textwidth}
	\highlight{Appropriate evaluation is crucial to not only promote the healthy development of FL, but the evaluations themselves can enable further applications.}
	\begin{itemize}
		\item Evaluation as Quality Control.
		\item Evaluation for Incentive Design.
		\item Evaluation as Online Verification.
	\end{itemize}
\end{minipage}}

\vspace{0.1cm}
Paragraph 5.

\fbox{\begin{minipage}{0.9\textwidth}
	\highlight{In contrast, the inappropriate evaluation will produce biased assessments, and the undiscovered limitations in FL algorithms or systems will damage real-world applications. For example, undiscovered privacy vulnerabilities will not only leak data providers' privacy but also decrease people's trust and willingness to further contribute data in the federated systems; FL algorithms untested under different data distributions may achieve poor model quality in applications as the data distribution in real-world applications can be highly heterogeneous~\cite{zhao2018federated,li2021fedbn,yang2021achieving,sattler2019robust,jeong2018communication,li2019convergence,DBLP:conf/iclr/YangFL21,DBLP:conf/iclr/LiJZKD21}; FL systems not evaluated on real-world network conditions may fail to achieve expected efficiency in applications due to the limited bandwidth and high latency in real-world applications.}
\end{minipage}}

%%%%%%%%%%%%%
\vspace{0.5cm}
\noindent
\underline{\textbf{Comment 3:}} \textbf{The authors over-emphasize the "standard" evaluation metrics. Instead, "standardizing" the procedure to obtain these metrics is more important than just "standardizing" the metrics. Indeed, the metrics are important, but the metrics obtained from different testbeds or scenarios can be varied, so there is no need to compare them. Accordingly, it is meaningful to compare the metrics that are obtained in the same testbed or scenario.}

\vspace{0.3cm}
\noindent
\underline{\textbf{Response:}} Thanks for your valuable suggestion. We highly agree with the reviewer's comment that standardizing the metrics is the first step, and it is more important to standardize the procedure to obtain these metrics. The ideal testbed for FL evaluation is using physical edge devices (\eg, smartphones), which is costly for researchers and problematic in scalability when dealing with hundreds or thousands of clients. A practical and widely used testbed is simulating a bunch of clients using computing servers. Thus, compared with conventional machine learning, the major challenge of obtaining standard FL evaluation metrics is how to appropriately simulate heterogeneous clients and capture metrics (\eg, communication costs) that reflect real-world conditions. To solve this challenge, we propose FedEval, which has a well-designed simulator for participants and their communications and obtains metrics close to real-world scenarios. Specifically:

\begin{itemize}
    \item Producing standard evaluation results requires a proper simulation for participants and communication between them. A widely-used method for simulating multiple participants is using multiprocessing, but we think it has the following problems: 1) it is hard to control the hardware resources (\eg, CPU and memory) used by each process; 2) it is hard to evaluate the performance under different network settings (i.e., bandwidth and latency). Our solution is putting all the participants into different docker containers, in which the hardware resources used by each participant could be fully controlled, including the CPU, GPU, memory, disk storage, \etc. The communication between containers is bridged by container networks. Thus, it is easy to change the network settings (\ie, bandwidth and latency).
    \item Measuring the communication size properly is also challenging. Many existing FL studies obtain communication size by directly measuring the size of the transmitted objects through utility packages like "getsizeof()". However, such evaluation has two issues: 1) different packages usually have different results; 2) not all the objects could be accurately assessed using this method. To solve these problems, we measure the communication size by directly collecting data from the virtual network interface card (NIC), which automatically records the amount of data sent out and received. Our solution is more accurate and significantly reduces the implementation complexity.
\end{itemize}

With appropriate client simulation, resource control, and communication measurements, the other metrics could be easily obtained in a standardized manner. For example, the time evaluation could be done using different timestamps (\eg, timestamps of receiving and uploading the model updates), and evaluating stragglers by allocating clients with heterogeneous computing or networking resources. 

In summary, we really appreciate the reviewer's comment and have significantly revised the paper about obtaining standardized evaluation results. Apart from the metrics and measures, we emphasize the process of obtaining these metrics, since metrics obtained from different testbeds or scenarios can be varied. To address this challenge, FedEval carefully simulates clients and their communication, and each device's computational and networking resources could be customized to simulate real-world scenarios. Our evaluation results are obtained under such a standard process instead of collecting evaluation results from the origin paper, which precisely matches the reviewer's comment about comparing metrics obtained in the same testbed or scenarios.


\vspace{0.3cm}
\noindent
The corresponding revision of this comment in \Cref*{sec:fedeval}:
\begin{mdframed}[style=2]
	\highlight{
	Compared with conventional machine learning, the major challenge of obtaining standard FL evaluation metrics is how to appropriately simulate heterogeneous clients and capture metrics (\eg, communication costs) that reflect real-world conditions. We introduce the FedEval platform's approach to addressing this challenge.
	\begin{itemize}
		\item Participants and Network Simulation. A widely-used method for simulating multiple participants is using multiprocessing, but we think it has the following problems: 1) it is hard to control the hardware resources (\eg, CPU and memory) used by each process; 2) it is hard to evaluate the performance under different network settings (\ie, bandwidth and latency). Our solution is putting all the participants into different docker containers, in which the hardware resources used by each participant could be fully controlled, including the CPU, GPU, memory, disk storage, \etc. The server and clients from different containers communicate through WebSocket. Container networks bridge the communication between containers. Under such an architecture design, it is easy to change the network settings (\ie, bandwidth and latency) by directly configuring the virtual network interface card (NIC).
		\item Communication Evaluation. Communication size is an essential evaluation metric for FL algorithms since the participants in FL tend to have limited network bandwidth, and a large communication size may bring significant efficiency overhead. A naive solution for evaluating the communication size, which is used in many existing FL studies, is directly measuring the size of the transmitted objects in the memory, and many utility packages (\eg, the "getsizeof()" function in Python) could be used. However, such evaluation implementation may have two issues: 1) Different packages usually have different results; 2) Not all the objects could be accurately assessed using this method. To solve these problems, we measure the communication size by directly collecting data from the virtual NIC, which automatically records the amount of data sent out and received. Compared with measuring the transmitted data size in memory, our solution is more accurate and significantly reduces the implementation complexity.
	\end{itemize}
	With appropriate client simulation, resource control, and communication measurements, the other metrics could be easily obtained. For example, the time evaluation could be done using different timestamps (\eg, timestamps of receiving and uploading the model updates), and the straggler evaluation in the utility could also be done by allocating clients with heterogeneous computing or networking resources.
	}

	\dots
	
	\highlight{In summary, FedEval provides a flexible framework for researchers to produce standardized evaluation results that closely mimic real-world settings using the measurements summarized in this survey.} \dots
\end{mdframed}

% %%%%%%%%%%%%%
\vspace{0.5cm}
\noindent
\underline{\textbf{Comment 4:}} \textbf{In section III-A, the definitions of FE, LE, and CE lack justification and there is insufficient experimental validation to support the rationale of these definitions. Similarly, while Figure 4 implies the aforementioned definitions for goals like effectiveness and robustness, there is a lack of necessary explanations. This raises doubts among readers regarding the validity of this open-source platform.}

\vspace{0.3cm}
\noindent
\underline{\textbf{Response:}} Thanks for your valuable suggestion. This comment contains multiple sub-questions, and we address them one by one.

\vspace{0.3cm}
\noindent
(A) \textbf{Comment 4.1: In section III-A, the definitions of FE, LE, and CE lack justification and there is insufficient experimental validation to support the rationale of these definitions.} 

In \Cref*{sec:goals}, we explain the rationale for definitions of FE, LE, and CE. We analyze the difference in utility definition between conventional machine learning and FL, give two possible utility definitions for FE and LE, and explain why we chose one instead of the other. Specifically, the following revisions are made to \Cref*{sec:goals}:
\begin{mdframed}[style=2]
\highlight{The definition of central effectiveness (\ie, \Cref*{def:CE}) follows accuracy definition from conventional machine learning, \ie, the ratio of correctly predicted samples in the whole evaluation dataset \cite{james2013introduction}. While the definitions of local effectiveness (LE) and FL effectiveness (FE) are more complicated since the data is distributed across the clients. Empirically, we can compute the effectiveness of each client and then aggregate all clients' results \cite{DBLP:conf/nips/LinHLZ22,DBLP:conf/nips/Yu0K0J22,li2019fair,DBLP:conf/icml/LubanaTKDM22,NEURIPS2020_24389bfe,DBLP:conf/icml/PillutlaMMRS022,DBLP:conf/icml/LinCX0GD022,jeong2022factorized,li2022soteriafl,alam2022fedrolex,DBLP:conf/icml/ChenHLCX0Z23,liu2022privacy,pmlr-v202-li23o,pmlr-v202-mai23b,pmlr-v202-baek23a,pmlr-v202-wu23z,pmlr-v202-zhang23aa}. One problem is how to set the aggregation weights, which intuitively have two approaches: uniform weights or weighted by the number of samples. Very few studies explain which approach they use in the evaluation, but we see both types of implementations when investigating the open-sourced code on GitHub (\eg, \cite{DBLP:conf/nips/LinHLZ22}\footnote{\url{https://github.com/desternylin/perfed}} used weights by sample and \cite{DBLP:conf/nips/Yu0K0J22}\footnote{\url{https://github.com/yaodongyu/TCT}} used uniform weights). Theoretically, these two types of weights are identical if all clients hold the same number of samples. However, the number of data samples held by each client could be very heterogeneous in real-world applications, making these two weights produce incompatible results. In this survey, we recommend using weights by the number of samples, the reasons are 1) weights by the number of samples matches the loss of FL \cite{mcmahan2017communication}, which is also weighted averaged by the number of training samples; 2) uniform weights could produce biased evaluation since the clients with very small amount of data may dominate the final accuracy; If the system is specifically optimized for clients with small amount of data, we recommend to report effectiveness for these clients separately, instead of mixing with other rich-data clients.}
\end{mdframed}

In summary, we define CE following conventional machine learning methods, discuss two possible approaches to defining FE and LE, and choose one as our final definition based on a deep understanding of the difference between these two approaches.
\vspace{0.2cm}

In \Cref*{sec:fedeval}, we add experimental validation to support the rationale of the CE, LE, and FE definitions (\ie, $LE < FE < LE$). We report utility evaluation results of four FL algorithms (\ie, FedSGD, FedAvg, FedProx, and FedOpt) on four datasets, and \Cref{tab:utility evaluation response} shows the results. The experimental results demonstrate the correlation of $LE < FE < LE$, which shows the rationale of the definition. Specifically, the evaluation shows that all the tested FL algorithms are able to achieve better utility than local training and show small decreases in utility compared to centralized training (\ie, the upper bound). Regarding the robustness, FedProx achieves the best performance, which also matches the original paper.

\begin{table}[h]
	\setlength{\tabcolsep}{0.3em}
	\renewcommand\arraystretch{0.7}
	\caption{Utility evaluation of four popular FL methods through FedEval on four datasets. All the experiments are repeated ten times, and the average values and standard error (\ie, values in parentheses) are reported.}
	\label{tab:utility evaluation response}
	\centering
	\begin{threeparttable}
	\begin{tabular}{c|c|c|c|c|c|c|c}
		\toprule
		Dataset & IID & LE & CE & FedSGD(FE) & FedAvg(FE) & FedProx(FE) & FedOpt(FE)  \\
		\midrule
		mnist   & N & \multirow{3}{*}{\tabincell{c}{0.11319\\(0.013)}}  & \multirow{3}{*}{\tabincell{c}{0.98614\\(0.001)}} & \tabincell{c}{0.98390\\(0.001)} & \tabincell{c}{0.97843 \\ (0.006)} & \tabincell{c}{0.97874\\(0.003)} & \tabincell{c}{0.97679\\(0.003)} \\
		\cmidrule(l){1-2}
		\cmidrule(l){5-8}
		mnist   & Y &  &  & \tabincell{c}{0.98341\\(0.002)} & \tabincell{c}{0.98651\\(0.001)} & \tabincell{c}{0.98683\\(0.001)} &  \tabincell{c}{0.98351\\(0.001)} \\
		\midrule
		femnist & N & \multirow{3}{*}{\tabincell{c}{0.48231\\(0.056)}} & \multirow{3}{*}{\tabincell{c}{0.84961\\(0.002)}} & \tabincell{c}{0.80461\\(0.015)} & \tabincell{c}{0.81234\\(0.004)} & \tabincell{c}{0.81288\\(0.005)} & \tabincell{c}{0.80783\\(0.003)} \\
		\cmidrule(l){1-2}
		\cmidrule(l){5-8}
		femnist & Y &  &  & \tabincell{c}{0.81351\\(0.012)} & \tabincell{c}{0.83476\\(0.004)} & \tabincell{c}{0.83385\\(0.002)} & \tabincell{c}{0.83187\\(0.004)} \\
		\midrule
		celebA  & N & \multirow{3}{*}{\tabincell{c}{0.70307\\(0.007)}} & \multirow{3}{*}{\tabincell{c}{0.92400\\(0.005)}} & \tabincell{c}{0.91707\\(0.005)} & \tabincell{c}{0.90170\\(0.005)} & \tabincell{c}{0.90120\\(0.007)} & \tabincell{c}{0.89913\\(0.008)} \\
		\cmidrule(l){1-2}
		\cmidrule(l){5-8}
		celebA  & Y &  &  & \tabincell{c}{0.91867\\(0.006)} & \tabincell{c}{0.90267\\(0.012)} & \tabincell{c}{0.90210\\(0.011)} & \tabincell{c}{0.89957\\(0.011)} \\
		\midrule
		sent140 & N & \multirow{3}{*}{\tabincell{c}{0.74447\\(0.006)}} & \multirow{3}{*}{\tabincell{c}{0.79263\\(0.002)}} & \tabincell{c}{0.74131\\(0.006)} & \tabincell{c}{0.75578\\(0.003)} & \tabincell{c}{0.75626\\(0.003)} & \tabincell{c}{0.75263\\(0.004)} \\
		\cmidrule(l){1-2}
		\cmidrule(l){5-8}
		sent140 & Y &  &  & \tabincell{c}{0.74024\\(0.005)} & \tabincell{c}{0.76504\\(0.004)} & \tabincell{c}{0.75839\\(0.005)} & \tabincell{c}{0.74955\\(0.007)} \\
		\midrule
		Average & N & \multirow{3}{*}{\tabincell{c}{0.51076}} & \multirow{3}{*}{\tabincell{c}{0.88809}} & \tabincell{c}{0.86172} & \tabincell{c}{0.86206} & \tabincell{c}{0.86227} & \tabincell{c}{0.85909} \\
		\cmidrule(l){1-2}
		\cmidrule(l){5-8}
		Average & Y &  &  & \tabincell{c}{0.86395} & \tabincell{c}{0.87224} & \tabincell{c}{0.87029} & \tabincell{c}{0.86612} \\
		\bottomrule
	\end{tabular}
    \end{threeparttable}
\end{table}

\vspace{0.3cm}
\noindent
(B) \textbf{Comment 4.2: Figure 4 implies the aforementioned definitions for goals like effectiveness and robustness, there is a lack of necessary explanations.} In \Cref*{sec:fedeval}, we enrich the explanation of \Cref*{fig:rader_charts} regarding the definition and computation methods of goals like effectiveness and robustness. Specifically, \Cref*{fig:rader_charts} delivers a straightforward overview of the evaluation results to identify the strengths and weaknesses of FL algorithms. Creating the radar charts is challenging since we need to reasonably organize different goals with disparate units and scales into the exact figure. Next, we introduce computation methods for \Cref*{fig:rader_charts}.

\begin{figure*}[h]
	\center
	\begin{subfigure}[t]{0.22\textwidth}
		\includegraphics[width=\textwidth]{figures/FedSGD_radar} 
	\end{subfigure} \hspace{+1mm}
	\begin{subfigure}[t]{0.22\textwidth}
		\includegraphics[width=\textwidth]{figures/FedAvg_radar}
	\end{subfigure} \hspace{+1mm}
	\begin{subfigure}[t]{0.22\textwidth}
		\includegraphics[width=\textwidth]{figures/FedProx_radar}
	\end{subfigure} \hspace{+1mm}
	\begin{subfigure}[t]{0.22\textwidth}
		\includegraphics[width=\textwidth]{figures/FedOpt_radar}
	\end{subfigure}
	\caption{(\ie, \Cref*{fig:rader_charts} in the paper) Visualizing the FedEval evaluation results through radar charts which compare four most popular FL algorithms from security and privacy, utility (\ie, robustness and effectiveness), and efficiency (\ie, communication and time consumption).}
	\label{fig:rader_charts response}
	\vspace{-2mm}
\end{figure*}

\begin{itemize}
	\item Efficiency score (quantitative). The efficiency score is calculated by averaging the quantitative score of three sub-metrics: communication rounds, communication amount, and time consumption. For each of these sub-metrics, we choose one baseline model, score 1 point to the baseline model, and then compute the score of other methods by comparing it to the baseline model. Denote $P_a$ as the method A's performance, $P_b$ as the performance of the baseline model, $\bar{P}$ as the ideal best performance. We set FedSGD as the baseline mode. We set the best performance $\bar{P}=0$ for time consumption, $\bar{P}=1$ for communication rounds, and $\bar{P}=0$ for communication amount. The scoring schema is shown in the following table.
	\begin{longtable}{p{4cm}|p{6cm}}
		\toprule
		Continues Score & Scoring Schema \\\midrule
		$0 \sim 1$ if $P_a \le P_b$ & $e^{1-P_b/P_a}$ \\\midrule
		$1 \sim 5$ if $P_a > P_b$ & $1 + 4(P_b - P_a)/(P_b - \bar{P})$ \\\bottomrule
	\end{longtable}
	\item Robustness score (quantitative). The robustness score consists of two parts: robustness under heterogeneous data and system. Regarding heterogeneous data, we give $3 \sim 1$ scores when the non-IID performance ($FE_{non-iid}$) disparity to the IID model $FE_{iid}$ is $1\% \sim 5\%$ accordingly. Regarding performance under the heterogeneous system, we temporarily use discrete scores (\ie, 1 or 0) to represent whether the algorithm properly handles the stragglers and dropouts or not.
	\begin{longtable}{p{3cm}|p{8cm}}
		\toprule
		Discrete Score & Scoring Schema \\\midrule
		0 & $||FE_{iid}-FE_{non-iid}||/||FE_{iid}|| > 5\%$ \\\midrule
		1 & $5\% \ge ||FE_{iid}-FE_{non-iid}||/||FE_{iid}|| > 3\%$ \\\midrule
		2 & $3\% \ge ||FE_{iid}-FE_{non-iid}||/||FE_{iid}|| > 1\%$ \\\midrule
		3 & $1\% \ge ||FE_{iid}-FE_{non-iid}||/||FE_{iid}||$ \\\midrule
		+1 & If properly handles stragglers \\\midrule
		+1 & If properly handles dropouts \\\bottomrule
	\end{longtable}
	\item Effectiveness score (quantitative). If the model's performance is better than the local model, we score according to the performance disparity to the central model. Score $5 \sim 1$ if performance disparity to the central model is $\le 1\%$, $\le 3\%$, $\le 5\%$, $\le 10\%$, and $\le 20\%$, respectively. The algorithm has $0$ score if the performance is worse or equal to local training or significantly worse than central effectiveness.
	\begin{longtable}{p{3cm}|p{7cm}}
		\toprule
		Discrete Score & Scoring Schema \\\midrule
		0 & $FE \le LE$ or $||FE-CE||/||CE|| > 20\%$ \\\midrule
		1 & $20 \ge ||FE-CE||/||CE|| > 10\%$ \\\midrule
		2 & $10\% \ge ||FE-CE||/||CE|| > 5\%$ \\\midrule
		3 & $5\% \ge ||FE-CE||/||CE|| > 3\%$ \\\midrule
		4 & $3\% \ge ||FE-CE||/||CE|| > 1\%$ \\\midrule
		5 & $1\% \ge ||FE-CE||/||CE||$ \\\bottomrule
	\end{longtable}
	\item Security \& Privacy score (qualitative). For the privacy and security score, we temporarily use the qualitative measure in the radar chart and will update the charts as well as the computation methods when more attack experiments are conducted. Specifically, we categorize the ability to defend against privacy and security attacks into different levels based on the amount of information transmitted between the server and clients. For the ability to resist the privacy attack on the client side, if the clients send less information to the server, they have a stronger ability to defend against data privacy attacks. Specifically:
	\begin{longtable}{p{2cm}|p{8cm}}
		\toprule
		Discrete Score & Scoring Schema \\\midrule
		0 & if clients upload raw data \\\midrule
		1 & if clients upload gradients calculated from a single round of training \\\midrule
		2 & if clients upload gradients calculated from multiple rounds of training \\\midrule
		3 & if clients leverage DP as protection or the parameters are compressed \\\midrule
		4 & if clients leverage secure aggregation \\\midrule
		5 & if clients leverage HE as protection \\\bottomrule
	\end{longtable}
	For the ability to resist the model security attack on the server side, if the server receives more information, it has a stronger ability to defend against the model security attacks. Specifically: 
	\begin{longtable}{p{2cm}|p{8cm}}
		\toprule
		Discrete Score & Scoring Schema \\\midrule
		5 & if the server holds raw data and can always make sure the model is training on the real dataset \\\midrule
		4 & if the server receives updates calculated from a single round of training \\\midrule
		3 & if the server receives updates calculated from multiple rounds of training \\\midrule
		2 & if the server only learns updates protected by DP or the parameters are compressed \\\midrule
		1 & if the server only learns aggregation results (\eg, secure aggregation) \\\midrule
		0 & if the server learns nothing (\eg, using HE) \\\bottomrule
	\end{longtable}
	It is worth noting that the above qualitative measure is only our temporary choice and will switch to quantitative measure when more attack experiments are conducted.
\end{itemize}

We put the detailed methods for obtaining the radar charts on an online document: \url{https://fedeval.readthedocs.io/en/latest/benchmark/benchmark.html#radar-chart}, which is provided in the paper. We will continue evaluating more algorithms and update the radar charts accordingly in the future, \ie, through online documents.

%%%%%%%%%%%%%
\vspace{0.5cm}
\noindent
\underline{\textbf{Comment 5:}} \textbf{The results in Figure 3 are unjustified. The authors claim that Figure 3 is based on the capability of the open-source platform proposed in this paper to evaluate the performance of FL algorithms. However, they do not mention whether there are comparable experimental results available in the original papers for these algorithms. In other words, there is no explanation or evidence provided to demonstrate the consistency between the results obtained in the original papers and the results obtained using the FedEval.}

\vspace{0.3cm}
\noindent
\underline{\textbf{Response:}} Thanks for your valuable suggestion. In \Cref*{sec:fedeval}, we add explanations to show that FedEval's evaluations match the conclusions from the original papers. Based on the evaluations in FedEval, the main conclusions from the original papers are correct and consistent. Specifically,

\begin{itemize}
	\item FedAvg \cite{mcmahan2017communication} focuses on improving efficiency by reducing the number of global communications and obtaining better efficiency than FedSGD. The efficiency evaluations in FedEval show that FedAvg has superior efficiency than FedSGD, which validates the conclusion of the original paper \cite{mcmahan2017communication}.
	\item FedOpt focuses on proposing federated optimizers (\eg, using momentums) to accelerate the federated training process. The efficiency evaluations in FedEval show that FedOpt has superior efficiency on the Shakespeare dataset, which matches the conclusion from the original paper. (Shakespeare is a relatively larger datasets that bring more efficiency overhead.)
	\item FedProx proposes to solve the non-IID problem by limiting clients' local updates such that the models trained on heterogeneous clients do not deviate significantly from the global model. The utility evaluations in FedEval show that FedProx has better performance regarding robustness, which matches the conclusion in \cite{fedprox}. 
\end{itemize}

We evaluate these algorithms using FedEval rather than collecting results from the original paper because the results from different papers are obtained using different testbeds or scenarios. FedEval can produce standardized evaluation results that are close to real-world scenarios, producing comparable evaluation results for FL studies across different times and research directions.

%%%%%%%%%%%%%
\vspace{0.5cm}
\noindent
\underline{\textbf{Comment 6:}} \textbf{There are still format issues in the manuscript.
- The arrangement of each subsection in Section III is messy. For instance, in Section Ill-A, the definition part, bold part, and existing work part are formatted differently, which looks disorganized and lacks logical order.
- The equation writing is unprofessional, such as the multiplication in formula (1), $p_kF k (w)$ should be replaced with $p_k \cdot F _k (w)$. The writing should be polished carefully.
- Several tables are not clearly listed. It would be better to put the system name for each work in Tables I-III. Also, it is difficult to identify the characteristics of each work. I highly suggest the authors enlarge the table line space or reorganize the tables.}


\vspace{0.3cm}
\noindent
\underline{\textbf{Response:}} Thanks for your valuable suggestion. This comment contains several sub-questions, and we address them one by one.

\vspace{0.3cm}
\noindent \textbf{(A) Comment 6.1: The arrangement of each subsection in Section III is messy. For instance, in Section Ill-A, the definition part, bold part, and existing work part are formatted differently, which looks disorganized and lacks logical order.} We reorganize \Cref*{sec:measure} and remove unnecessary bold texts to be clear. After the reorganization, the \Cref*{sec:measure} is organized as following:

\vspace{0.3cm}
\begin{mdframed}[style=2]\highlight{
\noindent
III Federated Learning Evaluation Measures (Section)
\begin{itemize}
	\item A Utility Evaluation Measures (Subsection)
		\begin{itemize}
		\item Effectiveness (Bold)
		\item Robustness (Bold)
		\item Existing Works on Utility Evaluation (Bold)
		\end{itemize}
	\item B Efficiency evaluation measures (Subsection)
		\begin{itemize}
		\item Communication (Bold)
		\item Computation (Bold)
		\item Existing Works on Efficiency Evaluation (Bold)
		\end{itemize}
	\item C Security \& Privacy Evaluation Measures (Subsection)
		\begin{itemize}
		\item \lbrack Data Privacy\rbrack \  Data Reconstruction Attack (Bold)
		\item \lbrack Data Privacy\rbrack \  Inference Attack (Bold)
		\item \lbrack Data Privacy\rbrack \  ID Leakage (Bold)
		\item \lbrack Model Security\rbrack \  Byzantine Attacks (Bold)
		\item \lbrack Model Security\rbrack \  Backdoor Attacks (Bold)
		\item Threat Model (Bold)
		\item Existing Works on Security \& Privacy Evaluation (Bold)
		\end{itemize}
\end{itemize}
}\end{mdframed}
\vspace{0.3cm}

\noindent \textbf{(B) Comment 6.2: The equation writing is unprofessional, such as the multiplication in formula (1), $p_kF k (w)$ should be replaced with $p_k \cdot F _k (w)$. The writing should be polished carefully.} Thanks for the reviewer's detailed comment. We have corrected the formula and carefully checked all the other formulas. We also have carefully checked the writing of the whole paper and corrected the grammar issues and unclear representations.

\vspace{0.3cm}
\noindent \textbf{(C) Comment 6.3: Several tables are not clearly listed. It would be better to put the system name for each work in Tables I-III. Also, it is difficult to identify the characteristics of each work. I highly suggest the authors enlarge the table line space or reorganize the tables.} We update \Cref*{tab:utility,tab:privacy,tab:efficiency metrics} to make them clearer to read. The changes include: 1) adding the system name, primitive design goals, and keywords of each paper to make it easier to identify the characteristics of each work; 2) enlarging the line spacing to make it easier to read. Specifically, \Cref{fig:tab} shows the enriched system name, primitive goals, and keywords.

\begin{figure*}[h!]
	\centering
	\includegraphics[width=.9\linewidth]{response_letter_figure/table_1.pdf}
	\caption{Following the reviewer's comment, we add the system name, primitive design goal (\ie, summarized from the papers' abstract and introduction), and keywords to better identify the characteristics of each work. We use the authors' names as substitutes if the paper does provide a system name. We also enlarge the table line space to make it easy to read.}
	\label{fig:tab}
\end{figure*}

%%%%%%%%%%%%%
\vspace{0.3cm}
\noindent
\underline{\textbf{Comment 7:}} The writing can be improved, as several quite long sentences exist in this manuscript. It would be better to break them into short ones. Also, several grammar errors should be corrected. For example,
-P4 Line 16: "i.e.,," should be "i.e.,";
-P11 Line 30: "FL platforms means"-> "FL platforms mean"
- In the last paragraph of Section I and in Section V-E, "etc" is written in italics. However, in the rest of the manuscript, "etc" appears in regular font style. The same issue also occurs with "e.g.". It not only lacks consistency in font style but also appears with double commas, such as "e.g.,,"
Please carefully proofread the manuscript and correct them all.

\vspace{0.3cm}
\noindent
\underline{\textbf{Response:}} Thanks for your valuable suggestion. We have corrected all the issues in the comment and carefully checked the overall writing of the paper to fix the grammar issues and the unclear representations.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Rewiewer 3
\section{Response to reviewer 3}

%%%%%%%%%%%%%
\vspace{0.3cm}
\noindent
\underline{\textbf{Comment 1:}} As a survey, there is a slight lack of content and the contribution is somewhat inadequate. Furthermore, the opensource platform, FedEval, proposed in this paper has already been extensively discussed in another paper by the author. Is it appropriate to mention it again as one of the contributions of this paper?

\vspace{0.3cm}
\noindent
\underline{\textbf{Response:}} Thanks for your valuable suggestion. We intend to make FedEval (\ie, the open-sourced platform) a contribution to this paper, and will not prepare another publication. We enrich the contents of FedEval, which are discussed in response to Comment 2. Overall, we enhance the following parts of the survey to enrich the content and highlight the contribution. Specifically,

\begin{itemize}
	\item \Cref*{sec:introduction}. We highlight the importance of an appropriate evaluation in FL. Specifically, FL is an interdisciplinary field with multiple optimization objectives. Researchers from different areas usually only focus improvements and evaluations on aspects they care about. However, in FL, the goals from these different areas are often interrelated, \ie, improving one goal can negatively impact other goals \cite{NFL-1,NFL-2}. Therefore, we urgently need a survey to summarize these objectives, analyze the tradeoffs among them, and ensure the healthy development of research in the FL field. Additionally, we demonstrate the issues caused by inappropriate evaluations in real-world applications.
	\item \Cref*{sec:goals}. Apart from introducing the evaluation goals one by one, we enrich the analysis of trade-offs between different goals and explicitly explain the necessity of doing a comprehensive evaluation, which is largely overlooked by existing studies. Specifically, 1) comprehensive analysis is the foundation of a fair comparison, and 2) comprehensive analysis is the key to finding all the limitations before being applied in real-world applications. We also propose solutions to reduce the workload of comprehensive evaluations: 1) We provide an easy-to-use evaluation platform with built-in evaluation goals and measures to reduce the workload; 2) For incremental methods that only improve one or two goals based on an existing solution, another option is to analyze that the remaining goals have identical performance to prior studies that already reported comprehensive evaluation results. With these enriched contents, we provide a more clear demonstration of the importance of comprehensive evaluations and how to perform comprehensive evaluations.
	\item \Cref*{sec:fedeval}. We enrich the contents of FedEval, including the methods of simulating the participants and different network conditions, the method for measuring the communication amounts, and additional experimental results on utility and security \& privacy.
\end{itemize}

With these enriched contents, we believe this survey can provide a comprehensive overview of the evaluation goals and measures and provide a useful reference for future efforts in advancing FL evaluation.

%%%%%%%%%%%%%
\vspace{0.5cm}
\noindent
\underline{\textbf{Comment 2:}} \textbf{If another paper on FedEval is not intended for formal publication but rather as a contribution to this paper, the description of this platform in this paper may be deemed insufficient. For instance, both Figure 3 and Figure 4 lack essential elucidations.}

\vspace{0.3cm}
\noindent
\underline{\textbf{Response:}} Thanks for your valuable suggestion. We will not consider another formal publication for FedEval and consider this platform as a contribution to this survey. We have enriched the contents about the platform as well as explanations of results in Figure 3 and Figure 4. Specifically:

In \Cref*{sec:fedeval}, we introduce FedEval's solution of obtaining standardized and comparable evaluation results. Specifically, compared with conventional machine learning, the major challenge of obtaining standardized and comparable FL evaluation results is appropriately simulating heterogeneous clients and capturing metrics (e.g., communication costs) that reflect real-world conditions. FedEval puts clients into different docker containers and enables control of each client's computational and communication resources to produce standardized evaluation results under various real-world application scenarios. The following revisions are made to the paper:

\begin{mdframed}[style=2]
	\highlight{
	Compared with conventional machine learning, the major challenge of obtaining standard FL evaluation metrics is how to appropriately simulate heterogeneous clients and capture metrics (\eg, communication costs) that reflect real-world conditions. We introduce the FedEval platform's approach to addressing this challenge.
	\begin{itemize}
		\item Participants and Network Simulation. A widely-used method for simulating multiple participants is using multiprocessing, but we think it has the following problems: 1) it is hard to control the hardware resources (\eg, CPU and memory) used by each process; 2) it is hard to evaluate the performance under different network settings (\ie, bandwidth and latency). Our solution is putting all the participants into different docker containers, in which the hardware resources used by each participant could be fully controlled, including the CPU, GPU, memory, disk storage, \etc. The server and clients from different containers communicate through WebSocket. Container networks bridge the communication between containers. Under such an architecture design, it is easy to change the network settings (\ie, bandwidth and latency) by directly configuring the virtual network interface card (NIC).
		\item Communication Evaluation. Communication size is an essential evaluation metric for FL algorithms since the participants in FL tend to have limited network bandwidth, and a large communication size may bring significant efficiency overhead. A naive solution for evaluating the communication size, which is used in many existing FL studies, is directly measuring the size of the transmitted objects in the memory, and many utility packages (\eg, the "getsizeof()" function in Python) could be used. However, such evaluation implementation may have two issues: 1) Different packages usually have different results; 2) Not all the objects could be accurately assessed using this method. To solve these problems, we measure the communication size by directly collecting data from the virtual NIC, which automatically records the amount of data sent out and received. Compared with measuring the transmitted data size in memory, our solution is more accurate and significantly reduces the implementation complexity.
	\end{itemize}
	With appropriate client simulation, resource control, and communication measurements, the other metrics could be easily obtained. For example, the time evaluation could be done using different timestamps (\eg, timestamps of receiving and uploading the model updates), and the straggler evaluation in the utility could also be done by allocating clients with heterogeneous computing or networking resources.
	}
\end{mdframed}

In \Cref*{sec:fedeval}, apart from the original efficiency (\Cref*{fig:fedeval_efficiency_evaluation}) and radar charts (\Cref*{fig:rader_charts}), we add utility (\Cref*{tab:utility evaluation}) and privacy \& security evaluations (\Cref*{fig:comparing fedsgd and fedavg on DLG}). We enrich explanations for all the evaluations, including a detailed analysis of the results, comparing the results obtained from FedEval with the original paper, and detailed methods for obtaining the evaluations. The following revisions are made to the paper:

\begin{mdframed}[style=2]
	An important characteristic of FedEval is its capability to evaluate an FL algorithm's performance from a holistic perspective including utility, efficiency, and security \& privacy. We have tested representative FL algorithms, including FedSGD~\cite{mcmahan2017communication}, FedAvg~\cite{mcmahan2017communication}, FedProx~\cite{fedprox}, FedOpt~\cite{reddi2020adaptive}, \etc. \highlight{\Cref*{tab:utility evaluation} shows the utility evaluation of these four algorithms, \ie, comparing the effectiveness to local and central training and the effectiveness under non-IID data. The utility evaluation shows that all the tested FL algorithms have significantly better performance than local training and show a small decrease in accuracy compared to centralized training on most datasets. Regarding the robustness under non-IID data setting, FedProx has the best performance and yields the best average effectiveness under non-IID data, which matches the results reported from the original paper.} \Cref*{fig:fedeval_efficiency_evaluation} shows the efficiency comparison of these four algorithms regarding the communication rounds, communication amounts, and time consumption. \highlight{The efficiency evaluation shows that FedSGD tends to have worse efficiency compared to the other three algorithms, and FedOpt shows superior efficiency on a relatively large dataset (\ie, Shakespeare), which also matches the results report from the original paper.} \highlight{\Cref*{fig:comparing fedsgd and fedavg on DLG} shows the data reconstruction attack \cite{NEURIPS2019_60a6c400} between FedSGD and FedAvg. Theoretically, FedProx and FedOpt have the same attack results as FedAvg since clients in these protocols upload the same information (\ie, parameters after multiple rounds of local updates) to the server. \Cref*{fig:comparing fedsgd and fedavg on DLG} shows that FedAvg has better performance than FedSGD. The possible reason is that the parameters uploaded in FedAvg contain multiple rounds of local training while FedSGD only has one round of training, and the accumulated local updates in the parameters make it harder to recover the raw data.}

	\highlight{While the above table and figures independently present the evaluation results regarding utility, efficiency, and privacy, we also attempt to merge the evaluation results into one radar chat to provide an overview as well as highlight the strengths and weaknesses of each algorithm. The final results are presented in Figure~\ref{fig:rader_charts}. We put the detailed methods for obtaining the radar charts on an online document\footnote{\url{https://fedeval.readthedocs.io/en/latest/benchmark/benchmark.html}} due to the space limitation and ease of future updates, \ie, we will also continue evaluating more algorithms and the radar charts may also be updated accordingly. For more detail of FedEval, \eg, the interface design, please refer to our technical report \cite{chai2020fedeval} as well as the online document\footnote{\url{https://fedeval.readthedocs.io/}}.}
\end{mdframed}

%%%%%%%%%%%%%
\vspace{0.5cm}
\noindent
\underline{\textbf{Comment 3:}} \textbf{Most of the figures and tables in the paper lack necessary explanations, such as the meaning of black and white dots in the table, as well as a brief description of the structure of each part in the figures.}

\vspace{0.3cm}
\noindent
\underline{\textbf{Response:}} Thanks for your valuable suggestion. We have carefully checked all the figures and tables and added necessary explanations in the caption or the paper. Next, we list all the figures and tables with enriched explanations. 


\begin{longtable}{|p{2.8cm}|p{5cm}|p{7cm}|}
	\caption{Explanations of all figures/tables before and after the revision.}
	\label{tab:table caption}\\\hline
	Figure / Table & Before (Caption) & After Revision (Caption) \\\hline
	\Cref*{fig:evaluation} & An overview of FL evaluation goals and measures. & \highlight{An overview of FL evaluation goals and measures. Briefly, we categorize the evaluation goals of FL into three types: security \& privacy, utility, and efficiency (Section II). Then, we summarize how to measure these goals in detail (Section III).}\\\hline
	\Cref*{tab:utility} & Utility evaluations in recent representative FL papers. & \highlight{Utility evaluations in recent representative FL papers. To better identify the characteristics of each work, we present the papers' system names, primitive design goals, and keywords, which are summarized based on the papers' abstract and introduction. We use the authors' names as substitutes if the paper does provide a system name (\eg, \citet{DBLP:conf/ccs/PasquiniFA22}). In the table, the black and white dots indicate whether the research work considers the corresponding measurements in the evaluation or not, which is investigated from the evaluation sections of the paper.}\\\hline
	\Cref*{tab:efficiency metrics} & Efficiency evaluations in existing works. $O(*)$ is the computation complexity analysis. & \highlight{Efficiency evaluations in existing works. $O(*)$ is the computation complexity analysis. Black dots indicate that a given study incorporated the corresponding measure in its evaluation, while white dots denote that the paper did not include that measure. Meanwhile, we also summarize the scale of efficiency evaluation in different studies, represented by the number of clients.} \\\hline
	\Cref*{tab:privacy} & Privacy evaluations in existing works. & \highlight{Privacy evaluations in existing works. Similarly, the black and white dots represent whether the studies considered the corresponding measures in the evaluation or not, respectively. Regarding the security definition, we also summarize the threat models used in representative works (\ie, semi-honest, malicious, or not defined in the paper).} \\\hline
	\Cref*{fig:bm_system_framework} & An overview of the FedEval evaluation platform. & \highlight{Users can evaluate existing algorithms using preset datasets in FedEval under different scenarios by providing the data, model, and runtime configs. Users can also evaluate new algorithms on new datasets by customizing the data, model, and strategy modules. Using the built-in evaluation goals and measures, FedEval significantly reduces the workload of the FL evaluation and produces standardized evaluation results.} \\\hline
	\Cref*{fig:fedeval_efficiency_evaluation} & Efficiency evaluation of four popular FL methods through FedEval. & \highlight{Efficiency evaluation of four popular FL methods through FedEval on four datasets. The results show that FedSGD has the worst efficiency regarding both communications and computations, and FedOpt has superior efficiency on the larger datasets (\ie, Shakespeare), which match the results reported by original papers.} \\\hline
	\Cref*{fig:comparing fedsgd and fedavg on DLG} & (New Figure) & \highlight{FedSGD vs. FedAvg under the data-reconstruction attack. FedAvg has better performance than FedSGD by having lower attack label accuracy and higher L2 distance between the recovered and real samples.} \\\hline
	\Cref*{tab:utility evaluation} & (New Table) & \highlight{Utility evaluation of four popular FL methods through FedEval on four datasets. All the experiments are repeated ten times, and the average values and standard error (\ie, values in parentheses) are reported. The MNIST dataset adopts the non-IID label setting, while the other datasets adopt the non-IID feature settings.} \\\hline
\end{longtable}



==> sections/response_minor.tex <==
\noindent
\textbf{Paper}: TKDE-2023-08-1161

\noindent
\textbf{Title}: A Survey for Federated Learning Evaluations: Goals and Measures

\noindent
\textbf{Authors}: Di Chai, Leye Wang, Liu Yang, Junxue Zhang, Kai Chen, and Qiang Yang

\vspace{0.5cm}

\noindent
Dear Editor and Reviewers,

\vspace{0.25cm}
\noindent
Thanks for your insightful and constructive comments and advice. We have carefully addressed these concerns and appropriately revised the manuscript. These comments and suggestions have enabled us to provide a highly improved manuscript. We really appreciate your help in processing this paper, and we are looking forward to hearing from you soon.

\vspace{0.25cm}
\noindent
Yours sincerely,

%\vspace{0.2cm}
\noindent
Di Chai and Leye Wang

\vspace{0.2cm}
\noindent \rule[1px]{6cm}{0.05em}
\vspace{0.2cm}

\noindent
Below, we first summarize all changes made to the manuscript in the revision. Then, we list all the responses to the comments made by each reviewer.

\section*{Summary of Changes} 
% \begin{cmt*}{}{}
% Editor Comments.
% \end{cmt*}

% \vspace{0.1cm}
% \noindent
% \underline{\textbf{Response:}}
% \vspace{0.2cm}

% Your response. 

\vspace{0.3cm}
\noindent \Cref*{sec:fedeval} - FedEval: A platform for FL System Evaluation
\vspace{0.1cm}
\begin{enumerate}
    \item \highlight{Enrich the description of FedEval's implementation.}
    \item \highlight{Demonstrate the workflow of evaluating customized FL algorithms.}
	\item \highlight{Demonstrate the workflow of evaluating privacy \& security attacks and the corresponding defending methods.}
\end{enumerate}

\vspace{0.3cm}
\noindent Appendices
\vspace{0.1cm}
\begin{enumerate}
    \item \highlight{Add full descriptions of FedEval's function interfaces.}
    \item \highlight{Discuss the extensibility of FedEval to evaluate different FL platforms.}
\end{enumerate}

% \fbox{\begin{minipage}{0.9\textwidth}\revision{Evaluation plays a critical role in designing various FL algorithms and systems, owing to the need for rigorous performance assessment, providing comparative analysis between different algorithms, ensuring robustness across diverse environments, and identifying limitations for further improvement.}\end{minipage}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Rewiewer 1
\section{Response to Reviewer 1} 

%%%%%%%%%%%%%
\noindent
\underline{\textbf{Comment 1:}} \textbf{I think the description of FedEval is still a little inadequate.}

\vspace{0.3cm}
\noindent
\underline{\textbf{Response:}} Thanks for your valuable suggestion. We have enriched the description of FedEval from two aspects: 1) the implementation of FedEval, and 2) the usage of FedEval to evaluate customized algorithms. 

Regarding the implementation of FedEval, we add the implementation detail of the time evaluation, which is challenging because it may have many variations based on different purposes. Specifically, apart from the overall time consumption in each training round, we would like to provide many other time consumption statistics to help the researchers improve the FL algorithms. For example, the computation and communication time at the clients, and the aggregation time at the server. The naive implementation of these time evaluation metrics is complicated and requires significant modifications to the source code. In FedEval, our idea is to collect a group of well-designed timestamps through which various time evaluation metrics could be flexibly calculated.

Notably, after enriching the implementation detail of the time evaluation, we have solved all the challenges regarding appropriately simulating the clients and capturing metrics that reflect real-world conditions. Specifically, as demonstrated in the paper, we simulate different clients using isolated containers which makes it easy to control the computation and communication resources of each client; we collect communication metrics directly from virtual NIC; we collect multiple rounds of well-designed timestamps which can support computing various time metrics. Regarding the utility, FedEval strictly follows the measurements in \Cref*{sec:measure} which are also widely used by existing work. Regarding security \& privacy, we provide flexible callback functions to implement various attacking and defending algorithms, which will be introduced next.

Regarding the usage of FedEval to evaluate customized FL algorithms as well as the attacking and defending methods, we add \Cref{fig:illustration_example_appendix} to make a clear demonstration. Specifically, FedEval provides a group of well-designed strategy functions to control the workflow of FL algorithms, \eg, customizing the aggregation function and local training algorithms. Meanwhile, FedEval provides a group of callback functions to implement various attack and defending methods, \eg, researchers can use the callback function to poison the data before local training. We provide a full list and description of FedEval's function interface in Appendix~\ref*{appendix:interface}.

\begin{figure*}[ht]
	\centering
	\includegraphics[width=.9\linewidth]{figures/illustration_example.pdf}
	\caption{\highlight{The FedEval's detailed workflow when evaluating customized algorithms. Users can provide scripts encompassing different strategy functions, enabling the assessment of various customized algorithms. For instance, these functions can customize the aggregation of parameters and the process of updating the global parameters to the local models. Additionally, users can test diverse attacking and defending techniques through different callback functions. As illustrated, clients can perform customizable data poisoning prior to local training and model poisoning before uploading updates. Conversely, the server can execute customizable data-revealing attacks and defend against poisoning attacks originating from the client side. We put the full description of the function interface of FedEval in Appendix~\ref*{appendix:interface}.}}
	\label{fig:illustration_example_appendix}
\end{figure*}

We also discuss the extensibility of FedEval to evaluate different FL platforms in Appendix~\ref*{appendix:evaluate platform}. Specifically, we can use the same goals and measures, containing the privacy, robustness, effectiveness, and efficiency metrics, to evaluate FL platforms. Furthermore, regarding the evaluation platform, we can integrate different FL platforms as different backends (\ie, the execution layer) and provide a hyper-parameter for users to determine which platforms (\eg, FedScale) will be used in the evaluation. We treat the detailed evaluation metric design and evaluation platform implementation for evaluating the FL platforms as our future work, and we believe such an evaluation will significantly benefit the FL studies.

The corresponding revision of this comment:

\vspace{0.2cm}
\noindent
\Cref*{sec:fedeval}

\begin{mdframed}[style=2]\highlight{
Time Evaluation. The implementation of time evaluation in FL is challenging because it may have many variations based on different purposes. For example, apart from the overall time consumption in each training round, we would also like to provide other time consumption statistics to help the users improve the FL algorithms, \eg, the computation and communication time of the clients, the aggregation time at the server, \etc. The naive implementation of these time evaluation metrics is complicated and requires significant modifications to the platform's source code. Our solution is providing a flexible time evaluation by collecting a group of timestamps, through which multiple time evaluation metrics could be calculated. Specifically, as illustrated in \Cref{fig:illustration_example}, we put four timestamps in the platform, which are the time of server sends parameters ($t_1$), clients receive parameters ($t_2$), clients send parameters ($t_3$), and server receives parameters ($t_4$). Assuming we have $k$ clients in the training, then $\{ (t_1^i, t_2^i, t_3^i, t_4^i) | 1 \le i \le k \}_n$ represents all the timestamps collected in the $i$-th round. Different combinations of these timestamps have different meanings:
\begin{itemize}
	\item Client computation time (average): $\frac{1}{k}\sum_{i=1}^k (t_3^i - t_2^i)$.
	\item Server aggregation time in the $n$-th round:\\ $sa=min(\{t_1^i | 1 \le i \le k \}_n)-max(\{t_4^i | 1 \le i \le k \}_{n+1})$
	\item Real-world time consumption in the $n$-th round:\\ $min(\{t_1^i | 1 \le i \le k \}_n)-min(\{t_1^i | 1 \le i \le k \}_{n+1})$
	\item Federated time consumption in the $n$-th round:\\ $sa + max(\{t_4^i-t_1^i | 1 \le i \le k \}_{n})$
\end{itemize}
}\end{mdframed}

\begin{mdframed}[style=2]\highlight{
To demonstrate the usability of FedEval, we present its detailed workflow when evaluating customized algorithms in \Cref{fig:illustration_example_appendix}. As illustrated in the figure, the researchers can provide strategy functions to customize the behaviors of the FL algorithm, \eg, how the parameters are aggregated at the server and how to set the global updates to the local model. Meanwhile, the researchers can use customized callback functions to perform experiments of attacking and defending against the attacks. On the client side, we can use callback functions to poison the data before local training or poison the model before uploading local updates. On the server side, we can use callback functions to perform data-revealing attacks when receiving individual client updates and detect the poisoning updates before the aggregation. Due to the space limitation, we put the full description of the function interface of FedEval in Appendix~\ref*{appendix:interface}.
}\end{mdframed}

\vspace{0.1cm}
\noindent
\Cref*{sec:future directions}

\begin{mdframed}[style=2]\highlight{
Notably, we can extend the evaluation goals and measures in this survey from evaluating algorithms into platforms, containing utility, security \& privacy, and efficiency. We discuss the extensibility of FedEval to evaluate different FL platforms in Appendix~\ref*{appendix:evaluate platform}.
}\end{mdframed}

% \vspace{0.1cm}
% \noindent
% Appendices

% \begin{mdframed}[style=2]
% \input{sections/appendix.tex}
% \end{mdframed}
